Target Set Selection Parameterized by Clique-Width and Maximum Threshold

The Target Set Selection problem takes as an input a graph $G$ and a non-negative integer threshold $ \mbox{thr}(v) $ for every vertex $v$. A vertex $v$ can get active as soon as at least $ \mbox{thr}(v) $ of its neighbors have been activated. The objective is to select a smallest possible initial set of vertices, the target set, whose activation eventually leads to the activation of all vertices in the graph. We show that Target Set Selection is in FPT when parameterized with the combined parameters clique-width of the graph and the maximum threshold value. This generalizes all previous FPT-membership results for the parameterization by maximum threshold, and thereby solves an open question from the literature. We stress that the time complexity of our algorithm is surprisingly well-behaved and grows only single-exponentially in the parameters.

==> structural-parameters.tex <==


%---------------------------------------------------------------------
%---------------------------------------------------------------------
\section{Constant TSS parameterized by Cliquewidth}

%---------------------------------------------------------------------
\subsection{Preliminaries}

Key ideas:
\begin{itemize}
	\item Dynamic Programming approach based on the clique-decomposition.
	\item There are classes of threshold, original threshold, color and reachability of color \( \times \) threshold that the class cannot be connected to.
	\item Remember required amounts for each class with reachability constraints.
	\item Remember for the not connected vertices, their threshold.
	\item Any connection condition may occur at most \( \tmax \) often.
\end{itemize}

\begin{definition}
	Let \( \GG \) be a graph with thresholds and \( S \subseteq V(G) \). Then,
	\begin{align*}
		& \newa{0}{\GG} \; := \; \bigset{ v \in V }{ \thr(v) = 0 }, \\
		& \newa{i}{\GG} \; := \; \bigsetcolon{ v \in V }{ | N(v) \cap \newa{<i}{\GG} | \geq \thr(v) } \\
		& \newa{< i}{\GG} \; := \; \bigcup_{ i' < i } \newa{i}{\GG},
	\end{align*}
	Let \( \GG_S \) be \( \GG \) but with threshold \( \thr_S: V \to  \N, \thr_S(v) \mapsto \begin{cases}
			0, & V \in S \\
			\thr_{\GG}(v), & V \notin S
	\end{cases} \).\\
	Then, \( S \) is a target set of \( \GG \) if \( V(G) = \newa{\infty}{\GG_S} := \bigcup_{i \in \N} \newa{i}{\GG_S} \).
\end{definition}

\begin{definition}
	A directed graph \( H \) on \( V(G) \) is
	an \define{activation graph} of \( (G,\thr) \) if it is acyclic and for all vertices \( v \in V(G) \) we have \( d^-_H(v) \geq \thr(v) \).
\end{definition}

\begin{lemma}[\cite{CombinatorialModelAndBoundsForTSS2010}]
	Let \( G \) be a graph with thresholds \( \thr: V \mapsto \N \) and \( S \subseteq V(G) \).
	There is an activation graph of \( (G,\thr_S) \) if and only if \( S \) is a target set of \( (G,\thr) \).
\end{lemma}

\begin{itemize}
	\item clique-decomposition
	\begin{itemize}
		\item \( (\alpha,a) \) introducing an isolated vertex with color \( \alpha \) and threshold \( a \).
		\item \( f_1 \oplus f_2 \): Disjoint union of \( \graph(f_1) \) and \( \graph(f_2) \).
		\item \( \eta_{\alpha, \beta} f' \), for \( \alpha \neq \beta \):
		``Join''
		Adding \textbf{e}dges to all nodes labeled \( \alpha \), nodes labeled \( \beta \) combinations. 
		\item \( \rho_{\alpha \to \beta} f' \): \textbf{R}e-labeling \( \alpha \) to \( \beta \).
	\end{itemize}
\end{itemize}

%---------------------------------------------------------------------
\subsection{Activation of Complete Bipartite Graphs}

There is an order of the initial points so that we can add edges from the start to all of the other side which are allowed.

\begin{definition}
	Let \( \GG \) be a graph with coloring and thresholds.
	Let \( \thr \) be defined by \( \partm \), that is for \( \thr(v) = \thr( \partm(v) ) \).
	Let \( \hgraph \) be a directed subgraph of \( \GG \).
	Let \( \GG \) have a complete subgraph between vertex sets \( A, B \subseteq V(\GG) \), that define sizes
		\( \amax := \min\{ \tmax(\GG), |A| \} \), \( \bmax := \min\{ \tmax(\GG), |B| \} \) and \( s := \amax + \bmax \).
	Let \( \VV_{A,B} \) be the family of vectors of vertices \( V_{A,B} \subseteq  A \cup B \) with \( |V_{A,B} \cap A| = \amax \) and \( |V_{A,B} \cap B| = \bmax \).
	
	Let \( V_{A,B} = ( v_i, \dots, v_s ) \in \VV_{A,B} \).
	For every vertex \( v_i \in A \), let \( E(v_i) := \{v_i\} \times B \setminus \bigcup_{i' <  i} v_{i'} \),
	likewise for \( v_i \in B \), let \( E(v_i) := \{v_i\} \times A \setminus \bigcup_{i' <  i} v_{i'} \),	
	 let \( E(V_{A,B}) \) be the union of edges \( \bigcup_{i \in [s]} E(v_i) \).
\end{definition}

\begin{definition}
	Let \( f \) be a clique-decomposition of \( \GG \).
	We denote by \( \KK_f \) be list of all \( \{A,B\} \) that occur as an edge-operation \( \eta_{\alpha,\beta} f' \) with \( A = V_\alpha ( \graph(f') ) \) and \( B = V_\beta ( \graph(f') ) \) in \( f \), ordered by the occurring in \( f \).
	%
	An directed acyclic subgraph \( \hgraph \) is \define{nice to \( f \)} if,
	for every \( \{A,B\} \in \KK := \KK_f \) there are vertices \( V_{A,B} \in \VV_{A,B} \),
	such that
	\( \hgraph = \bigcup_{ \{A,B\} \in \KK } E(V_{A,B})\).
\end{definition}

\begin{definition}
	Let \( f \) be a clique-decomposition of colored threshold-graph \( \GG \).
	Let \( \partm: V(\GG) \to \CC(\GG) \) be a class-mapping.
	Let \( \KK_1, \dots, \KK_z \) be the list of all pairs \( \{A,B\} \) that occur as an edge-operation \( \eta_{\alpha,\beta} f' \) with \( A = V_\alpha ( \graph(f') ) \) and \( B = V_\beta ( \graph(f') ) \) in \( f \), ordered by the occurring in \( f \).
	Let \( \KK_{\leq i} \) be the pairs \( \KK_1, \dots, \KK_i \).
	
	
	Let \( \hgraph' \) be an activation graph of \( \GG \) that is nice to \( f \) with \( V_{A,B}, \{A,B\} \in \KK \).
	For \( i \in [z] \), let \( \hgraph_i' := \bigcup_{ \{A,B\} \in \KK_{\leq i} } E( V_{A,B} ) \).
	Then
	%
	\[ \hgraph := \hgraph' \setminus \bigset{ (u,v) \in E( V_{\KK_i} ) }{ d^-_{\hgraph_i'}(v) \geq \thr( \partm(v) ), \; i \in [z] } \]
	
	 and \( \partm) \) are \define{nice} to \( f \).
\end{definition}

\begin{lemma}
\label{lemma:nice:activation:graph}
	Let \( G \) be a graph with thresholds \( \thr: V(G) \mapsto [0,\tmax] \) that activate the graph.
	Let \( f \) be a clique-decomposition of \( G \).
	There is an activation graph of \( \GG \) that is nice to \( f \).
\end{lemma}
\begin{proof}
	Let \( \KK := \KK_f \).
	We define \( \hgraph \) according to the following activation algorithm that assigns labels \( 1,\dots,|V(G)| \) to \( V \):
		Start with \( \hgraph = \emptyset \).
		Put all vetices \( v \) with \( d^-_H(v) \geq \thr(v) \) in a queue;
		remove the first vertex \( v \) of the queue assigning it the smallest free label;
		and add every edge \( (v,w) \) to \( \hgraph \) for which
			there is a pair of sets \( \{A,B\} \in \KK \) with \( (v,w) \in A \times B \)
				and \( w \) is not yet labeled
				and \( d^-_{\hgraph \cap (A \times B)}(w) < \tmax \).
				%and \( (w,v) \notin \hgraph \).	
	Repeat until the queue is empty.
	%The vertices according to the time-step they are removed from the queue.
	
	We show that the resulting \( \hgraph \) is an activation graph of \( (G,\thr) \).
	
	We show that \( \hgraph \) is circle-free.
	Assume, for the sake of contradiction, that there is a directed cycle \( C \) in \( \hgraph \).
	Then there is vertex \( w \) of the circle with the lowest label, and an ingoing edge \( (v,w) \in C \).
	Neighbor \( v \) has a higher label than \( w \).
	Contradiction to that only edges \( (v,w) \) where \( w \) has the higher label are added.
	
	We show that \( \hgraph \) activates every vertex.
	Assume, for the sake of contradiction, that \( w \) gets not activated, that is \( d^-_\hgraph(w) < \thr(w) \leq \tmax \) and \( \thr(w) \geq 1 \).
	Since, our activation-algorithm only adds edges from active vertices, for all neighbors \( v \) of \( w \) we have \( (w,v) \notin \hgraph \).
	Because the thresholds are activating, we have \( d^-_G(w) \geq \thr(w) \), and hence there is a neighbor \( v \) with \( (v,w) \notin \hgraph \).
	There is a pair \( \{A,B\} \in \KK \) with \( (v,w) \in \{A,B\} \).
	However, he algorithm did not add \( (v,w) \) when removing \( v \) from the queue.
	This means, that \( d^-_{\hgraph \cap K_{A,B}}(w) \geq \tmax \) or \( w \) has a lower label than \( v \).
	The later, that \( w \) has a lower label than \( v \), would imply that \( w \) has been added to the queue, and hence \( d_{\hgraph}^-(w) \geq \thr(w) \).
	Thus, the former is the case, that \( d^-_{\hgraph \cap (A \times B)}(w) \geq \tmax \).
	Therefore, \( d^-_{\hgraph}(w) \geq d^-_{\hgraph \cap (A \times B)}(w) \geq \tmax \thr(w) \) and \( w \) is activated by \( \hgraph \).
	Contradiction to the assumption that \( \hgraph \) does not activate \( w \).
	It follows, that \( \hgraph \) is an activation graph of \( (G,\thr) \).
	
	We claim that the resulting activation graph \( \hgraph \) is nice to \( f \).
	We identify an \( V_{A,B} \) for every \( \{A,B\} \in \KK \), and show that \( \hgraph = \bigcup_{ \{A,B\} \in \KK } E( V_{A,B} ) \).

	Let \( \{A,B\} \in \KK \).
	Let \( \amax = \min\{ \tmax, |A| \} \), \( \bmax = \min\{ \tmax, |B| \} \) and \( s = \amax + \bmax \).
	Let \( V_{A,B} = \{ v_1, \dots, v_{s} \} \) be the first \( \amax \) labeled vertices of \( A \) and the first \( \bmax \) labeled vertices of \( B \) ordered by increasing label.
	The greedy algorithm adds the following edges:
	For \( i \in [s] \), if \( v_i \in A \), edges \( v_i \) to \( B \setminus \bigcup_{i' <  i} v_{i'} \),
		if \( v_i \in B \), edges \( v_i \) to \( A \setminus \bigcup_{i' <  i} v_{i'} \).
	These are the edges \( E( V_{A,B} ) \).
	We therefore have that \( \hgraph \supseteq \bigcup_{ \{A,B\} \in \KK } E( V_{A,B} ) \).
	
	It remains to show that \( \hgraph \subseteq \bigcup_{ \{A,B\} \in \KK } E( V_{A,B} ) \)
	%for complete bipartite subgraph \( K_{A,B} \) is not part of \( E_{\hgraph, A, B} \).
	Assume, for the sake of contradiction, that there is an edge \( (u,v) \in \hgraph \) where, for every \( \{A,B\} \), we have \( (u,v) \notin E( V_{A,B} ) \).
	Then, the label of \( u \) is smaller than the label of \( v \).
	Further, there is at least one \( \{A,B\} \in \KK \) with \( (u,v) \in (A \times B) \) where \( d := d^-_{\hgraph \cap (A \times B)}(v) < \tmax \) just before \( (u,v) \) is added.
	Since in particular \( d = d^-_{\hgraph \cap (A \times B)}(v) < |A| \), we have that \( d \leq \amax \).
	%< \amax = \min\{ \tmax, |A| \} \) just before \( (u,v) \) is added.
	Further, \( u \) is the \( d \)th vertex of \( A \) that is removed from the queue.
	Therefore, \( u \in V_{A,B} \).
	Since the label of \( v \) is higher than the label of \( u \), we have that \( (u,v) \in E( V_{A,B} ) \).
	
	Hence, we have that \( \hgraph = \bigcup_{ \{A,B\} \in \KK } E( V_{A,B} ) \).
	It follows that \( \hgraph \) is nice to \( f \).
\end{proof}

\begin{lemma}
	Let \( f \) be a clique-decomposition of colored threshold-graph.
	There is an activation graph \( \hgraph \) of \( \GG \) and that \( \hgraph \) and the initial mapping \( \partm \) are nice to \( f \).
\end{lemma}
\begin{proof}
	\autoref{lemma:nice:activation:graph} gives us a nice activation graph \( \hgraph' \) of \( (G,\thr) \).
	Following the definition of a modest and nice activation graph, we remove edges.
	Thus, the resulting \( \hgraph \) is circle free.
	Further, only ingoing edges from \( v \) are removed, when an activation of \( v \) is still guaranteed.
	It follows that \( \hgraph \) is an activation graph of \( (G,\thr) \).
\end{proof}

%---------------------------------------------------------------------
\subsection{Nice Activation Graph}

\begin{definition}
	Let \( \GG \) be a graph with coloring and thresholds.
	Let \( \hgraph \) be a directed subgraph of \( \GG \).
	Let \( \GG \) have a complete subgraph between vertex sets \( A, B \subseteq V(\GG) \), that define sizes
		\( \amax := \min\{ \tmax(\GG), |A| \} \), \( \bmax := \min\{ \tmax(\GG), |B| \} \) and \( s := \amax + \bmax \).
	Let \( \VV_{A,B} \) be the family of vectors of vertices \( V_{A,B} = ( v_i, \dots, v_s ) \in A \cup B \) with \( |V_{A,B} \cap A| = \amax \) and \( |V_{A,B} \cap B| = \bmax \).
	
	
	
	For every \( V_{A,B} \in \VV_{A,B} \), let \( E(V_{A,B}) \) be the following set of edges:	
		For \( i \in [t] \), \( v_i \in A \), edges \( v_i \) to \( B \setminus \bigcup_{i' <  i} v_{i'} \);
		and for \( i \in [t] \), \( v_i \in B \), edges \( v_i \) to \( A \setminus \bigcup_{i' <  i} v_{i'} \).
\end{definition}

\begin{definition}
	Let \( \GG \) be a graph with coloring and thresholds, and \( f \) be a clique-decomposition of \( \GG \).
	We define \( \KK(f) := ( \KK_1(f), \dots, \KK_s(f) ) \) as the list of all tuples \( \{V_\alpha (\graph(F')), V_\beta (\graph(f'))\} \) whose colors occur as an edge-operation \( \eta_{\alpha,\beta} f' \) in \( f \), ordered by their occurring in \( f \).
	
	For \( \{A,B\} \in \KK (f) \), let \( \VV_{\{A,B\}} \) be the family of vectors of vertices \( V_{\{A,B\}} = ( v_i, \dots, v_s ) \in A \cup B \) with \( |V_{\{A,B\}} \cap A| = \amax \) and \( |V_{\{A,B\}} \cap B| = \bmax \).
	
	Let \( (V_1, \dots, V_s) \in ( \VV_1(f), \dots, \VV_s(f) ) \) be fixed.
	Let \( \hgraph^0 := \emptyset \).
	Let \( \hgraph^{i+1} \) the edges \( E(V_{i+1}) \) where their endpoint \( v \) has \( d^-_{\hgraph^{\leq i}}(v) < \thr(v) \).
	
	A directed subgraph \( \hgraph \) is \define{nice to \( f \)} if,
	for every \( \{A,B\} \in \KK(f) \) there are vertices \( V_{A,B} \in \VV_{A,B} \) such that
	\( \hgraph = \hgraph^1 \cup \dots \cup \hgraph^s \).
\end{definition}

BETTER:
Removing edges of \( \hgraph \) does not change whether its activating.

However, how do you show that \( \hgraph \) is nice? 
Maybe handle to many edges otherwise.

%---------------------------------------------------------------------
\subsection{Algorithm}

\begin{definition}
	Let \( \GG \) be a colored threshold-graph with colors \( [\ell] \) and thresholds of value at most \( \tmax \).
	%
	For every color \( \alpha \in [\ell] \), every \define{original threshold} \( \ao \in [0,\tmax] \) and every \define{current threshold} \( a \in [0,\ao] \), we define the \define{meta-class} \( \clA \).
	Let \( \col( \clA ) = \alpha \) be the color, \( \org( \clA ) = \ao \) be the original threshold, and \( \thr( \clA ) = a \) be the current threshold of meta-class \( \clA \).
	Further, \( \MM( \GG ) \) is the family of all meta-classes of \( \GG \), that is
	%
	\[ \MM ( \GG ) = \bigset{ \clA }{ \alpha \in [\ell], \; \ao \in [0,\tmax], \; a \in [0,\ao] } . \]
\end{definition}

\begin{observation}
	\( | \MM(\GG) | \leq \ell \cdot (\tmax+1)^2 \).
\end{observation}

\begin{definition}
	A class \( \cA \) of \( \GG \) is a cycle free subgraph of on \( \MM(\GG) \) that has a unique meta-class \( \rr(\cA) \), the \define{root}, that reaches all its contained meta-classes.
	Then, \( \CC( \GG ) \) be the set of classes of \( \GG \).
	
	Let \( \col(\cA) \) be the color of the root \( \rr(\cA) \), let \( \thr(\cA ) \) be the threshold-index of \( \rr(\cA) \) and \( \org(\cA) \) be the original threshold of \( \rr(\cA) \).
	For color \( \alpha \in [\ell] \) let \( \CC( \GG, \alpha ) \) be the classes of \( \CC(\GG) \) whose root has color \( \alpha \).
	For color \( \alpha \in [\ell] \) and original-threshold \( \ao \in [0,\tmax] \), let \(\CC(\GG, \alpha, \ao) \) be the family of all classes whose root has color \( \alpha \) and original-threshold \( \ao \).
\end{definition}

\begin{observation}
	\( | \CC | \leq 2^{|\MM|^2} = 2^{\ell^2 \cdot (\tmax+1)^4} \).
\end{observation}

\begin{definition}	
	For classes \( \cA, \cB \in \CC( \GG ) \), we define the partial ordering \( \cA \succeq \cB \) if the graph of \( \cB \) is an induced subgraph of the graph of \( \cA \).
	We write \( \cA \succ \cB \) if \( \cA \succeq \) and also \( \cA \neq \cB \).
	\footnote{In particular, just a (not-induced) subgraph is not sufficient.} %
	
	For a class \( \cA \in \CC(\GG) \) without meta-class \( \clC \in \MM(\GG) \), that is \( \clC \notin V(\cA) \),
		we define \( \cA[ \clC ] \) as the class \( \cA \) where the root \( \rr( \cA ) \) is replaced by \( \clC \).
	%
	Further, for incomparable classes \( \cB, \cBN \in \CC(\GG) \), let \( \cA[ \cBN / \cB] \) be the class \( \cA \) where the root of the subgraph \( \cB \), if it exists, is replaces by the root of \( \cBN \) with recursively outgoing edges as in \(  \cBN \).
\end{definition}

\begin{observation}
	
\end{observation}
\begin{proof}
	There, \( \clC \) is the new root, the former root \( \rr(\cA) \) is removed, and since \( \clC \notin V(\cA) \) the resulting directed graph is circle free.%
	\footnote{It is not useful to replace something other than the root, when only specifying the meta-class.
	The meta-class can occur as a non-root multiple times with different reachability.}
	%
	Because \( \cB, \cBN \) are incomparable, \( \cA[ \cBN / \cB] \) as well as \( \cA[ \cBN / \cB] \cup \cA \) are circle-free. 
	We freely use \( \cA \cup \cB \) to denote the joined edge sets of \( \cA \) and \( \cB \), given that \( \cA \cup \cB \) is circle-free and has a unique root.
	
	Let \( \cC[ \cBN / \cB, \AM ] \) be \( \cC[ \cBN / \cB] \) if \( \AM(\cB) = 0 \) and \( \cC[ \cBN / \cB ] \cup \cC \) if \( \AM(\cB) \geq 1 \).
\end{proof}

\begin{definition}
	Let \( \GG \) be a colored threshold-graph of colors \( [\ell], \ell \in \N \) and maximal threshold \( \tmax \).
	A mapping
	\[  \AM: \CC( \GG ) \to
		\begin{dcases}
			\{ \infty \} ,& |E(\cD)| = 0, \\
			 [0,\tmax] ,& |E(\cD)| \geq 1,
		\end{dcases}
	  \]
	are \define{amounts} of \( \GG \).
	Further, let 
	\( \thr( \cC ) \to [0, \org(\cC)] \) be the current threshold of \( \cC \).
\end{definition}	

\begin{observation}
\label{lemma:threshold:invariant:implies:threshold:cap}
	Let colored threshold-graph \( \GG \) have conditions \( \AM \) (not necessary with the \( \tmax \)-cap).
	Then for all non-trivial classes \( \cA, E(\cA) \neq \emptyset \) we have that \( \AM(\cA) \leq \tmax(\GG) \).
\end{observation}
\begin{proof}
	Let \( \cA \) be a non trivial class, that is \( E(\cA) \neq \emptyset \).
	Therefore, there is a child class \( \cA \succ_1 \cB \).
	Its amount \( \AM(\cB) \) is at most \( \sum_{\cC \succ_1 \cB} \AM(\cC) \).
	The threshold-invariant gives us that \(  \sum_{\cC \succ_1 \cB} \AM(\cC) \leq \org(\cB) - \thr(\cB) \leq \tmax(\GG) \).
	Thus, we have that \(\AM(\cA) \leq \tmax(\GG) \).
\end{proof}


\begin{definition}
	A mapping \( \partm : V(\GG) \to \CC(\GG) \) is a \define{class-mapping} if it is
	\begin{itemize}
		\item \contitle{\mappingPropertyDef} 
		for every vertex \( v \), its original threshold and color is preserved, that is \( \org(\partm(v)) = \thr(v) \) and  \( \col(\partm(v)) = \col(v) \).
	\end{itemize}	
	Class-mapping \( \partm \) \contitle{satisfies} amounts \( \AM \) of \( \GG \) if
		\amountPropertyDefText{\partm}.
		
	A \( k \)-activation graph \( \hgraph \) satisfying amounts \( \AM \) and \( f \)
		is a directed subgraph of \( \GG(f) \)
			such that there is a class-mapping \( \partm: V(\GG) \to \CC(\GG) \) satisfying \( \AM \) and
	\begin{itemize}
		\item \contitle{\hActivatingDef}
		there is a \( k \) vertex set \( S \) such that
			for every other vertex \( v \in V(\GG) \setminus S \) we have that \( d^-_\hgraph(v) = \thr( \partm(v) ) \),
		\item \contitle{\hAcyclicDef}
		\( \hgraph \cup \set{ (u,v) \in V^2 }{ \partm(u) \succ \partm(v) } \) is acyclic,
	\end{itemize}
\end{definition}

\begin{definition}
	A \( k \)-activation graph \( \hgraph \) satisfies \( f \) and \( \AM \) if
		there is a class-mapping \( \partm: V(\GG) \to \CC(\GG) \) such that
		\( \hgraph \) is nice to \( \partm \) and \( f \),
		and
		\( \hgraph \) satisfies amounts \( \AM \) with \( \partm \).
\end{definition}

\begin{definition}
	The conditions \( \AM \) of \( \GG \) where, for every \( \cA \in \CC(\GG) \)
	\[ \AM( \cA ) =
		\begin{cases}
			\infty, & \text{if } |V(\cD)| = 1, \; \org(\cA) = \thr(\cA) \text{ and }\\
			& \set{ v \in V(G) }{ \thr(v) = \thr(\cA) } \geq 1 \\
			0, & \text{else.}
		\end{cases}
	\]
	are the \define{initial conditions} of \( \GG \).
\end{definition}

	\begin{itemize}
		\item \( \AM(\cAN)+1 \leq \tmax \) as otherwise we can just add  \( \cAN \) to \( \cB \) the activating-property holds.
	\end{itemize}

\newcommand{\br}[1]{{\scriptstyle ( } #1 { \scriptstyle ) }}
\begin{definition}[Adding edges]
	\letABincomparable
	\begin{equation*}
	\cAN := \cA \cup \bigcup_{\cB \in \BB} \big( ( \rr \br{\cA}, \rr \br{\cB} ) \cup \cB \big),
	\end{equation*}
	For every class \( \cB \in \BB \), let \( \add{\cA, \cB}\thr(\cB) = \thr(\cB)-1\).
	%
	\[
		\def\arraystretch{1.1}
	    \add{\cA, \cB}\AM ( \cD ) =
	    \begin{dcases}
	    	\AM(\cAN) + 1						,& \cD = \cAN,  \\
	    	\AM( \cA )-1						,& \cD = \cA, \\	
 			%0									,& \cD \succ \cA \text{ and } \adjust(\cD) \neq \cD,\\
	        \AM( \cD )							,& \cD \notin \{\cA,\cAN\} . % \CC \text{ are all classes } \cC \in \adjust(\cD)^{-1} \setminus \{ \cD \} % \\
	        	        			 		%	& \text{with } \cC \succ \cA
	     \end{dcases}
	  \]
	are amounts of \( \GG \).
\end{definition}

\begin{definition}
	\letABincomparable
	Let \( \partm: V(\GG) \to \CC(\GG) \) and \( x \in \partm(\cA) \).
	Recall that \( \adjust(\cC) := \cC[ \cAN / \cA, \AM' ] [ \cBN / \cB ] \).
	We define the mapping \( \add{x,\beta} \partm: V(\GG) \to \CC(\GG) \) as
	%
	\begin{equation*}
		( \add{x,\beta} \partm  ) (v) :=
		\begin{dcases}
			\cAN 					,& v = x,\\
			\partm(v)				,& v \neq x.
		\end{dcases}
	\end{equation*}
	Let \( \partm^{-1}: V(\GG) \to \CC(\GG) \).
	\begin{equation*}
		( \deadd{x, \beta} \partm' )(v) :=
		\begin{cases}
			\cA			,& v = x, \\
			\partm'(v)	,& v \neq x.
		\end{cases}
	\end{equation*}
\end{definition}

\begin{lemma}
\label{lemma:one:fan:forward}
	\letABincomparable
	Let \( \partm: V(\GG) \to \CC(\GG) \), \( x \in \partm^{-1}(\cA) \), and \( X := \{ x \} \times \bigcup_{\cB \in \BB} \partm^{-1}(\cB) \).
	
	If \( k \)-activation graph \( \hgraph \supseteq X \) of \( \GG \) satisfies \( \AM \) with \( \partm \),
		then \( \hgraph \setminus X \) satisfies \( \add{ \cA, \cB } \AM \) with \( \add{ x, \cB} \partm \).
\end{lemma}

\begin{proof}
	For simplicity, let the new conditions be \( \AM' := \add{ \cA, \cB } \AM \) and \( \partm := \add{ x, \cB } \partm \).
	
	\begin{itemize}
		\item We show that \( \partm \) is a class-mapping.
		Every vertex \( v \in V(\GG) \) is mapped to a modified class \( \add{ x, \beta } \partm (v) \) with the same color and original threshold as the old class \( \partm(v) \).
		Since \( \partm \) satisfies the \proofbf{\mappingPropertyRef}, also \( \partm' \) satisfies the \mappingProperty.
	
		\item We show that \( \partm \) satisfies amounts \( \AM \), that \amountPropertyDefText{\partm'}.
		
		For \( \cC \notin \{\cA,\cAN\} \) we have \( x \notin \partm^{-1}(\cB) \) and thus \( \partm'^{-1}(\cB) = \partm^{-1}(\cB) = \AM(\cC) = \AM'(\cC) \).
		Else, for class \( \cAN \) we have that \( \partm'^{-1}(\cAN) = \partm^{-1}(\cAN)+1 = \AM(\cAN)+1 = \AM'(\cAN) \).
		And finally, for class \( \cA \) we have that \( \partm'^{-1}(\cA) = \partm^{-1}(\cA)-1 = \AM(\cA)-1 = \AM'(\cA) \).
		
		\item
		We show that \( \hgraph \setminus X \) is \hActivatingRef.
		That is, there is a \( k \)-vertex set \( S' \) such that for every other vertex \( v \in V(\GG) \setminus S \) we have that \( d_{\hgraph \setminus X}^- = \thr( \partm(v) ) \).
		We have that there is a \( k \)-vertex set \( S' \) such that for every other vertex \( v \in V(\GG) \setminus S \) we have that \( d_\hgraph^- = \thr( \partm(v) ) \).
		We show that \( \hgraph \setminus X \) is activating with set \( S \).
		
		\item
		It remains to show that \( \hgraph \setminus X \) satisfies the \proofbf{\hAcyclicRef}, that
			\( (\hgraph \setminus X) \cup \mappedpp \) with \( \mappedpp := \set{ (u,v) }{ \partm'(u) \succ \partm'(v) } \) is acyclic.
		Assume, for the sake of contradiction, that there is a cycle \( Q \) in \( (\hgraph \setminus X) \cup \mappedpp \).
		From this assumption we follow the contradiction that \( Q \) is also a cycle in \( \hgraph \cup \mappedp \) with \( \mappedp := \set{ (u,v) }{ \partm(u) \succ_1 \partm(v) } \).
		Every edge of \( Q \) from \( \hgraph \setminus X \) especially is in \( \hgraph \).
		It remains to show that every edge of \( \mappedpp \) also exists in \( \hgraph \cup \mappedp \).%
		\footnote{We may discuss transitivity of \( \succ \).}
		
		Case, \( \partm(u) = \cA \).
		Then \( \partm'(u) =  \cA[ \cBN / \cB ] \) or \( \partm'(u) = \cAN \).
		\begin{itemize}
			\item
			Consider that \( \partm'(u) = \cA[ \cBN / \cB ] \).
			Then \( \partm'(v) = \partm(v)[ \cBN / \cBN ] \).
			Because \( \partm(u)[ \cBN / \cB ] \succ_1 \partm(v)[ \cBN / \cB ] \) also \( \partm(u) \succ \partm(v) \).
			\item Otherwise \( \partm'(u) = \cAN \).
			If \( \partm'(v) = \cBN \), then \( (u,v) \in X \) and we are done.
			Else if \( \partm'(v) \neq \cBN \) we have that \( \cA[ \cBN / \cB ] \) has the children of \( \cAN \) but \( \cBN \).
			Hence \( \partm(u)[ \cBN / \cB ] \succ \adjust( \partm'(v) ) \).
			As \( \cB \nsucc \cA \) we have that \( \adjust( \partm'(v) ) = \partm'(v)[ \cBN / \cB ] \) and it follows that \( \partm(u) \succ \partm(v) \). 
		\end{itemize}
		
		Case, \( \partm(u) \neq \cA \) and \( \partm(v) = \cA \).
		Either \( \partm'(v) = \cA \) or \( \partm'(v) = \cAN \).
		
		\begin{itemize}
			\item
			Consider \( \partm'(v) = \cA \).
			Note that \( \partm'(u) = \partm(u)[ \cAN / \cA, \AM'][ \cBN / \cB ] \) cannot receive child \( \cA \) that \( \partm(u) \) does not have.
			Thus \( \partm(u) \succ_1 \partm(v) = \cA \).	
			\item
			Otherwise \( \partm'(v) = \cAN \). %meaning that \( v = x \).
			The \greedyPropertyRef applies for class \( \partm'(u) \neq \cA \) and color \( \alpha \).
			We have \( \alpha \)-colored \( \cAN, \cA \) with \( \cA \nsucc \partm'(u) \)
				as the contrary \( \cA \succ \partm'(u) \) implies the contradiction \( \cA \succ \partm'(u) \succ \partm'(v) = \cAN \). 
			Further \( \thr(\cAN) = \thr(\cA) \geq 1 \) and \( \AM(\cAN) \geq 1 \) (as \( \partm(u) \succ_1 \cAN \)), as well as \( \partm(u) \succ \cAN \).
			It follows that \( \partm(u) \succ \cA = \partm(v) \).
		\end{itemize}
	
		Case \( \partm(u) \neq \cA \neq \partm(v) \).
		Then \( \partm'(u) = \adjust(\cAN) \) and \( \partm'(v) = \adjust(\cBN) \).
		We have that \( \partm(u)[ \cAN / \cA, \AM' ] [ \cBN / \cB ] \succ \partm(v)[ \cAN / \cA, \AM' ] [ \cBN / \cB ] \) and therefore also that \( \partm(u) \succ \partm(v) \).	 
	\end{itemize}
\end{proof}	

\comment{
\begin{definition}
	Let \( \AM \) be conditions of colored threshold-graph \( \GG \).
	Let \( \partm': V(\GG) \to \CC(\GG) \) be a class-mapping.
	Let \( x \) be a vertex in \( \partm'^{-1}( \cAN ) \).
	Let \( Y \) be a set of \( \AM(\cB) \) many of \( \partm'^{-1}(\cBN) \).
	\begin{equation*}
		\partm(v) :=
		\begin{cases}
			\cA			,& v = x, \\
			\cAN		,& v \neq x, \; \partm'(x) = \cAN,\\
			\cB			,& v \in Y,\\
			\cBN		,& v \notin Y, \partm'( v ) = \cBN, \\
			\cC [ \cA / \cAN, \AM ] [\cB / \cB', \AM]	,& \partm'(v) = \cC \notin \{ \cAN, \cBN \}.
		\end{cases}
	\end{equation*}
\end{definition}}

\begin{lemma}
\label{lemma:one:fan:backward}
	\letABincomparable
	Let \( \partm': V(\GG) \to \CC(\GG) \), vertex \( x \in \partm'^{-1}( \cAN ) \) and \( X := \{ x \} \times \bigcup_{\cB \in \BB} \partm^{-1}( \cB ) \).
	
	If \( k \)-activation graph \( \hgraph' \) on \( \GG \setminus X \) satisfies \( \add{ \cA, \beta } \AM \) with \( \partm' \),
	 	then \( \hgraph' \cup X \) is a \( k \)-activation graph that satisfies \( \AM \) on \( \GG \) with \( \deadd{x,\beta} \partm' \).
\end{lemma}
\begin{proof}
	For simplicity, let \( G' = G-X \) and \( \AM' := \add{ \cA, \cB } \AM \).
	Let \( x \in \cAN \) be the one vertex such that \( X = \{x\} \times \partm^{-1}( \cBN ) \).
	
	\begin{itemize}
	\item
	We show that \( \deadd{x,\beta} \partm' \) is a class-mapping for \( \GG \).
	That is, for every vertex \( v \), its original threshold and color is preserved, formally \( \org((\partm(v)) = \thr(v) \) and \( \col(\partm(v)) = \col(v) \).
	We have that \( \org(\deadd{x,\beta} \partm'(v)) = \org(\partm'(v)) = \thr(v) \).
	Further, we have that \( \col( \deadd{x,\beta} \partm'(v) ) = \col( \partm'(v) ) = \col(v) \).
	
	\item
	We show that \( \deadd{x,\beta} \partm' \) satisfies amounts \( \AM \), that \amountPropertyDefText{ \deadd{x,\beta} \partm' }.
	\end{itemize}

	\ \\
	
	
	It remains to show that \( \hgraph \) satisfies the \proofbf{connectivity-condition}, that \( \hgraph \cup \mappedp \) is acyclic.
	Assume, for the sake of contradiction, that \( \hgraph \) contains a cycle.
	We show the contradiction that every edge of the cycle also exists in \( \hgraph \setminus X \cup \mappedpp \).
	For an edge in \( X \), say \( (x,y) \), we have \( \partm'(x) = \cAN \succ \cBN = \partm'(y) \), and hence \( (x,y) \in \mappedpp \).
	An edge \( \hgraph \setminus X \) trivially also exists in \( \hgraph \setminus X \cup \mappedpp \).
	It remains to show that every edge \( \mappedp \) also exists in \( \mappedpp \).
	...
\end{proof}


\begin{definition}
	Let \(  f = \eta_{\alpha,\beta} f' \) be a clique-decomposition of colored threshold-graph \( \GG \), that defines amounts \( \amax = \min\{ \tmax(f), |V_\alpha(\graph(f))| \} \) and \( \bmax = \min\{ \tmax(f), |V_\beta(\graph(f))| \} \) and \( s = \amax + \bmax \).
	A \define{class-vector} for colors \( \alpha, \beta \) and \( f \) is a list of classes \( \cC_1, \dots, \cC_s \in \CC(\graph(f)) \) of colors \( \gamma_1, \dots, \gamma_s \in \{\alpha,\beta\} \), where \( \amax \) are colored \( \alpha \) and \( \bmax \) are colored \( \beta \).
	We denote by \( \cvectorset( f ) \) every class-vector of colors \( \alpha, \beta \) and \( f \).
	Let \( \gamman_i := \{\alpha,\beta\} \setminus \gamma_i \) for \( i \in [s] \).
	For a class-vector \( \cvector \in \cvectorset(f) \), we define \( \add{ \cvector } \AM \) as
	%
	\[ {\add{ \cC_s, \gamman_s }} \dots {\add{ \cC_1, \gamman_1}} \AM . \]
	
	(2)
	Directed edge set \( \adde( \cvector ) \) is the union of \( \adde( \cC_i, \gamman_i) \) for all \( i \in [s] \).
	
	(3)
	Let \( \partm: V( \GG ) \to \CC( \GG ) \).
	Let vertices \( x_1, \dots, x_s \) be of color \( \gamma_1, \dots, \gamma_s \).
	We define \( \add{ x_1, \dots, x_s } \partm: V( \GG ) \to \CC( \GG ) \) as
	\[
		\big( \add{ x_1, \dots, x_s } \partm \big) (v) :=  {\add{ x_s, \gamman_s }} \dots {\add{ x_1, \gamman_1}} \partm (v) .
	\]
\end{definition}

\begin{observation}
	For a fixed clique-decomposition \( f \) and colores \( \alpha, \beta \), we have \( |\cvectorset(f)| \leq 2^{|\CC(\GG)|} \leq 2^{2^{\ell^2 \cdot (\tmax+1)^4}} \).
\end{observation}

\begin{lemma}
\label{lemma:join:forward}
	Let \(  f = \eta_{\alpha,\beta} f' \) be a clique-decomposition of colored threshold-graph, that has conditions \( \AM \).
	
	If there is a \( k \)-activation graph of \( \GG(f) \) satisfying \( f \) and \( \AM \),
		then
		for a class-vector \( \cvector \in \cvectorset(f) \)
		there is a \( k \)-activation graph of \( \GG(f') \) satisfying \( f' \) and \( \add{ \cvector }\AM \).
\end{lemma}
\begin{proof}
	For simplicity, let \( \GG := \graph(f) \), \( A = V_\alpha(\GG) \) and \( B = V_\beta(\GG) \).
		%\( A := \set{ a }{ \col(\partm(a)) = \alpha } \), \( B := \set{ b }{ \col(\partm(b)) = \beta }) \).
	Let \( \hgraph \) be a \( k \)-activation graph of \( \GG \) that is nice to \( f \) and \( \AM \)
		with class-mapping \( \partm: V(\GG) \to \CC(\GG) \).
	Since \( \hgraph \) is nice to \( f \) there is a list of vertices  \( V_{A,B} = v_1, \dots v_s \in A \cup B \) whose edges \( E(V_{A,B}) \) are the edges of the activation graph in \( A \times B \).
	Let \( \cvector = \cC_1, \dots \cC_s \) be the classes resulting from mapping each \( V_{A,B} \) to its class according to \( \partm \) adjusted by changes from adds.
	That is \( \cC_1 = \partm(v_1) \) and \( \cC_{i+1} = ( \add{ \cC_i, \dots, \cC_1 } \partm ) (v_{i+1}) \) for \( i \in [s-1] \).
	
	W.l.o.g.~\( \GG(f') \) does not have edges between \( A \) and \( B \).
	Thus \( \GG(f') \) is \( \GG(f) \setminus ( A \times B ) \).
	We show that \( \hgraph' := \hgraph \setminus (A \times B) \) is a \( k \)-activation graph of \( \GG(f') \) with class-mapping \( \add{ v_1, \dots, v_s } \partm \).
	Since \( \hgraph' \) is a subset of \( \hgraph \), it especially is also directed subgraph.
	
	Let \( X \) be the directed edges from one \( x \in \partm^{-1}( \cA ) \) to a all of vertices \( \partm^{-1}( \cB ) \) of color \( \col(\cB) = \beta \) with \( \AM(\cB) \geq 1 \) and \( \thr(\cB) \geq 1 \).
	We have that \( \AM(\cA) \geq 1 \) since \( x \in \partm(\cA) \) and \( \partm \) is a class-mapping.
	\autoref{lemma:one:fan:forward} shows that \( \hgraph \setminus X \) satisfies \( \add{ \cA, \beta }\AM \) on \( \GG - X \).
	Note that \( \add{ \cvector } \AM \) consecutively adds \( \add{ \cC_s, \gamman } \)...
	
	Therefore, \( \hgraph \setminus E(V_{A,B}) \) satisfies \( \add{ \cA, \cB} \AM \) on \( \GG - E(V_{A,B}) \).
	Since \( \hgraph \) is satisfies \( f \), we have that \( \hgraph \cap ( A \times B ) = E(V_{A,B}) \).
	Therefore \( \hgraph \setminus (A \times B) \) satisfies \( \add{ \class[\alpha,\beta] }\AM \)  on \( \GG(f') \).
	
	Observe, that if edges are not added, then only because \( \thr(\cB) = 0 \).
	It does not happen that \( \cB \) is a child of \( \cA \)
	
	We show that \( \hgraph \setminus (A \times B) \) satisfies \( f' \) and \( \add{ \cvector } \AM \) with \( \partm' = \add{ \cvector } \partm \).
	
\end{proof}

\begin{lemma}
\label{lemma:join:backward}
	Let \(  f = \eta_{\alpha,\beta} f' \) be a clique-decomposition of colored threshold-graph, and \( \AM \) be conditions of \( \graph(f) \).
	
	If for a class vector \( \cvector \in \cvectorset(f) \)
	there is a \( k \)-activation graph of \( \graph(f') \) that satisfies \( f' \) and \( \add{ \cvector }\AM \),
		there is a \( k \)-activation graph of \( \graph(f) \) that satisfies \( f \) and \( \AM \).
	%
	%For every class-vector \( \cvector \in \cvectorset \),
	%	if \( \hgraph \downharpoonright \graph(f') \) satisfies \( f' \) and \( \add( \cvector )\AM \),
	%	then \( \hgraph \) satisfies \( f \) and \( \AM \),
\end{lemma}
\begin{proof}
	For simplicity, let \( \GG' := \graph(f) \).
	Let \( \hgraph \) be a \( k \)-activation graph of \( \GG' \)

	Note, that \( \hgraph \downharpoonright \graph(f') \) is nice to \( f' \).

	Since \( \hgraph' \) is nice to \( f' \), to show that \( \hgraph' \cup E^{\alpha,\beta} \) is nice to \( f = \eta_{\alpha,\beta}f' \) it remains to show that \( (\hgraph' \cup E^{\alpha,\beta}) \cap (A \times B) = E^{\alpha,\beta} \). This is true since \( \hgraph' \cap (A \times B) = \emptyset \).
	
	Let \( X \) be the directed edges from one \( x \in \partm^{-1}( \cA ) \) to a class \( \cB \) of distinct colors.
	\autoref{lemma:one:fan:backward} shows that if \( \hgraph \setminus X \) satisfies \( \add{ \cA, \cB } \AM \) on \( \GG - X \), then \( \hgraph \) satisfies \( \AM \) on \( \GG \)
		...
	Therefore, \( \hgraph \cup E^{\alpha,\beta} \) satisfies \( \AM \) on \( \GG \).
\end{proof}

\begin{lemma}[Full Join]
	Let \(  f = \eta_{\alpha,\beta} f' \) be a clique-decomposition of colored threshold-graph \( \GG \), that has conditions \( \AM \).
	
	There is a \( k \)-activation graph that satisfies \( f \) and \( \AM \),
		if and only if
		there is a class-vector \( \cvector \in \cvectorset(f) \)
		such that
		there is a \( k \)-activation graph of \( \graph(f') \) that satisfies \( f' \) and \( \add{ \cvector }\AM \).
%		
%	Directed subgraph \( \hgraph \) of \( \graph(f) \) and class-mapping \( \partm: V(\GG) \to \CC(\GG) \) are nice to \( f \) and satisfy \( \AM \),
%		if and only if
%		there is a class-vector \( \cvector \in \cvectorset \)
%		such that
%		\( \hgraph \downharpoonright \graph(f') \) and class-mapping \( \add(\cvector) \) are nice to \( f' \) and satisfy \( \add( \cvector )\AM \).
\end{lemma}
\begin{proof}
	\forward
	This is proved in \autoref{lemma:join:forward}.
	
	\backward This is shown in \autoref{lemma:join:backward}.
\end{proof}

\begin{definition}
	Let clique-decomposition \( f = \eta_{\alpha,\beta} f' \) describe a colored threshold-graph, and \( \AM \) be conditions of \( \graph(f) \).
	%
	\[
		\opt( \; f, \; \AM \; ) \; := \; \min_{ \cvector \; \in \; \CC^{\alpha,\beta}( f ) } \opt( \; f', \; \add{ \cvector } \AM \; )
	\]
\end{definition}


\subsection{Partition}

\begin{definition}
	Let colored threshold-graph \( \GG \) have amounts \( \AM \).
	Let class \( \cA \in \CC(\GG) \) be of distinct color than \( \beta \in [\ell] \).
	Let \( \cB \) be the class \( \cA \) but where the root has color \( \beta \), and \( \AM(\cB) = 0 \).
	Let \( j \in [0, \AM(\cA) ] \).
	Let \( \partm: V(\GG) \to \CC(\GG) \) be a class-mapping.
	We define \( \partition( \cA, \beta, 0 ) \partm \) as \( \partm \).
	Otherwise we define \( \partition( \cA, \beta, j ) \) as follows.
	Let \( B \) be a subset of \( \partm^{-1}(\cA) \) of size \( j \).
	Then
	%
	\[
		\big( \partition( \cA, \beta, j)\partm \big)(v) :=
		\begin{dcases}
			\cA								,& \partm(v) = \cA, \; v \notin B, \\
			\cB								,& \partm(v) = \cA, \; v \in B, \\
			\partm(v)[ \cB / \cA, \AM' ]	,& \partm(v) \neq \cA.
		\end{dcases}
	\]
	%
	\[
	\big( \departition( \cA, \beta, j)\partm' \big)(v) := \partm(v)[ \cA / \cB ]
		%\begin{dcases}
		%	\cA						,& \partm'(v) \in \{ \cA, \cB \}, \\
		%	\partm(v)[ \cA / \cB ]	,& \partm'(v) \notin \{ \cA, \cB \}.
		%\end{dcases}
	\]
\end{definition}

\begin{observation}
	\( \partm = \departition( \cA, \beta, j) \partition( \cA, \beta, j) \partm \).
\end{observation}

\begin{definition}
	\introductionPartition
	We define \( \partition( \cA, \beta, 0 ) \AM \) as \( \AM \), and for \( j \geq 1 \) define \( \AM' := \partition( \cA, \beta, j ) \AM \) as follows.
	If \( V( \cA ) = 1 \),
	 let \( j' = \min\{ j , \AM(\cA) \} \) and \( i' \) be such that \( i' + j' = \AM( \cA ) \),
				else let \( i' = j' = \infty \).
	Then
	\begin{equation*}
		\big( \partition( \cA, \beta, j )\AM \big)( \cD ) =
		\begin{cases}
			i'						,& \cD = \cA \\
			j'						,& \cD = \cB \\
			\AM( \cC )	,& \cD = \cC[ \cB / \cA, \AM' ].
		\end{cases}
	\end{equation*}
	
	Let \( \alpha, \beta \in [\ell] \) be distinct colors.
	Let \( j: \CC(\GG, \alpha) \to [0,\tmax] \) be a mapping with \( \cA \mapsto [0, \AM(\cA)] \).
	Let \( \cA_1, \dots, \cA_s \) be all classes of \( \CC(\GG) \) of color \( \alpha \),
		and \( \cB_1, \dots, \cB_s \) be their respective classes where the root has color \( \beta \).
	Then \( \partition( \alpha, \beta, j ) \AM \) is
	%
	\[ \partition( \cA_1, \cB_1, j(\cA_1)) \dots \partition( \cA_s, \cB_s, j(\cA_s)) \AM \]
\end{definition}

\begin{lemma}
	%\introductionPartition
	%
	Then \( \partition( \cA, \beta, j )\AM \) are \amountsInfiniteRef and \greedyPropertyRef amounts of \( \GG \).
\end{lemma}
\begin{proof}
	Straight forward.
\end{proof}

\begin{lemma}
	\introductionPartition
	Let \( \GG \) be a graph, and \( \partm \) be a class-mapping satisfying \( \AM \).
	Let \( \GG' \) be the graph \( \GG \) where \( j \) many of \( \partm^{-1}( \cA) \) have color \( \beta \).
	
	Then \( \partition( \cA, \beta, j) \partm \) is a class-mapping of \( \GG' \) satisfying \( \partition( \cA, \beta, j )\AM \).
\end{lemma}
\begin{proof}
	We have to show that (1) \( \partm' := \partition( \cA, \beta, j) \partm \) preserves color and original threshold, and that (2) \( \partm' \) satisfies \( \AM' := \partition( \cA, \beta, j )\AM \).
	
	(1) Straight forward.
	
	(2) Straight forward.
\end{proof}

\begin{lemma}
	\introductionPartition
	
	Then \( \departition( \cA, \beta, j) \partm' \) is a class-mapping of \( \GG \) satisfying \( \AM \).
\end{lemma}
\begin{proof}
	We have to show that \( \partm := \departition( \cA, \beta) \partm' \) preserves color and original threshold, and that \( \partm \) satisfies \( \AM \).
	
	Straight forward.
\end{proof}

\begin{lemma}
	\introductionPartition
	
	If \( k \)-activation graph \( \hgraph \) of \( \GG \) satisfies conditions \( \AM \) with class-mapping \( \partm \), then \( \hgraph \) is a \( k \)-activation graph satisfying \( \partition(\cA,\beta,j) \AM \) with class-mapping \( (\partition( \cA, \beta, j )\partm \).
\end{lemma}
\begin{proof}
	We show that the \connectivityPropertyRef is true.
	Assume, for the sake of contradiction, that there is a cycle \( Q \) in \( \hgraph \cup \mappedpp \).
	We show that every edge in \( Q \) also exists in \( \hgraph \cup \mappedp \), which contradicts that \( \hgraph \) satisfies the \connectivityProperty.
	Trivially, edges in \( \hgraph \) are also in \( \hgraph \cup \mappedpp \).
	It remains to show that every edge \( (u,v) \) of \( \mappedpp \) also exist in \( \hgraph \cup \mappedpp \).
	
	Consider an edge from \( (u,v) \in \mappedpp \).
	The class \( \partm'(u) \) has child class \( \partm'(v) \).
	It follows that \( \partm(u) = \partm'[\cA / \cB](u) \) has child \( \partm(v) = \partm'[\cA / \cB](v) \).
	
	We show that \( \AM \) are \greedyPropertyRef.
	That is for every class \( \cD \) with \( \AM(\cD) \geq 1 \) and every monochromatic classes \( \cE, \cEN \) with \( \cEN \nsucc \cD \) and \( \thr( \cEN ) \geq 1 \), \( \AM( \cEN ) \geq 1 \), if \( \cD \succ \cE \) then \( \cD \succ \cEN \).
\end{proof}

\begin{lemma}
	Let \( f = \rho_{\alpha \to \beta} f' \) be a clique-decomposition of a colored threshold-graph, that has conditions \( \AM \).
	
	There is a \( k \)-activation graph satisfying \( f \) and \( \AM \)
		if and only if
		there is a mapping \( j: \; \CC( f, \alpha) \to [0,\tmax] \) and a \( k \)-activation graph satisfying \( f' \) and \( \partition( \alpha, \beta, j ) \AM \).	
\end{lemma}

\begin{definition}
	Let \( f = \rho_{\alpha \to \beta} f' \) be a clique-decomposition of a colored threshold-graph, that has conditions \( \AM \).
	%
	\[
		\opt( \; f, \; \AM \; ) \; = \; \minn{ j: \; \CC( f, \alpha) \to [0,\tmax(f)] } \opt( \; f', \; \partition( \alpha, \beta, j ) \AM \; )
	\]
\end{definition}

%-----------------------------------------------------------------------------------
\subsection{Forget}

\begin{definition}
	\introductionForget
	For class \( \cC \in \CC(\GG) \), let \( \forget{\cA} \cC \) be the graph as \( \cC \) without \( \cA \) where all predecessors of \( \cA \) are connected to all successors of \( \cA \).
	For non-trivial classes \( \cD \in \CC(\GG) \) let \( \forgetway{\cA} \cD \) be the unique class \( \cC \neq \cD, E(\cD) \neq \emptyset \) such that \( \forget{\cA} \cC = \cD \).
	It is not unique!
	\[
		\forget{\cA} \AM (\cD) := 
		\begin{dcases}
			\max \{ \AM( \cD ), \; \AM( \forgetway{\cA} \cD ) \} 		,& E(\cC) \neq \emptyset,\\
			\AM( \cD )													,& E(\cC) = \emptyset.
		\end{dcases} 
	\]
	\[
		\deforget{\cA} \AM( \cD ) :=
		\begin{dcases}
			\cC			,& \forgetway{\cA}(\cC) = \cD,\\
			\cD			,&	.
		\end{dcases}
	\]
\end{definition}

\begin{lemma}
	\introductionForget
	Then \( \forget{ \cA } \AM \) are amounts of \( \GG \).
\end{lemma}
\begin{proof}
	We show that \( \AM' := \forget{ \cA } \AM \) is well-defined
\end{proof}

\begin{lemma}
	\introductionForget
	
	If \( \partm \) satisfies \( \AM \), then \( \partm \downharpoonright  \) satisfies \( \forget{ \cA } \AM \).
\end{lemma}
\begin{proof}

\end{proof}

\begin{lemma}
	\introductionForget
	
	If \( \partm \downharpoonright  \) satisfies \( \forget{ \cA } \AM \), then \( \partm \) satisfies \( \AM \).
\end{lemma}

\begin{definition}
	Let \( f = f_1 \oplus f_2 \) be a clique-decomposition of colored threshold-graph, that has conditions \( \AM \).
	%
	\[
		\opt( \; f, \; \AM \; ) \; = \; \minn{ j,j': \; \CC(f) \to [0,\tmax(f)], \\ \text{for all } \cA \in \CC(f): \\ j(\cA) + j'(\cA) = \AM(\cA) } \opt( \; f_1, \; \partition( j ) \AM \; ) \; + \; \opt( \; f_2, \; \partition( j' ) \AM \; )
	\]
\end{definition}

\begin{lemma}
	Let \( f = (\alpha,a) \) be a clique-decomposition of a colored threshold-graph, that has conditions \( \AM \).
	
	There is a \( 0 \)-activation graph satisfying \( f \) and \( \AM \)
		if and only if
		there is \( \cA \in \CC \) with \( \thr(\cA) = 0 \) and \( \AM(\cA) = \infty \).
		
	There is an \( 1 \)-activation graph satisfying \( f \) and \( \AM \)
		if and only if
		there is \( \cA \in \CC \) with \( \thr(\cA) = 1 \) and \( \AM(\cA) = \infty \).
\end{lemma}
\begin{proof}
	To satisfy the matching conditions, a mapping \( \partm: V(\GG) \) has to map to \( \cA \) with \( \AM(\cA) = 1 \).
\end{proof}

\begin{definition}
	Let \( f = (\alpha,a) \) be a clique-decomposition of a colored threshold-graph, that has conditions \( \AM \).
	%
	\[
		\opt( \; f, \; \AM \; ) \; = \;
		\begin{dcases}
			0			,& \text{ there is } \cA \in \CC \text{ with } \thr(\cA) = 0 \text{ and } \AM(\cA) = \infty, \\
			1			,& \text{ there is } \cA \in \CC \text{ with } \thr(\cA) = 1 \text{ and } \AM(\cA) = \infty, \\
			\infty		,& \text{ else}.
		\end{dcases}
	\]
\end{definition}





